Improved search for $\psi(3770) \to \gamma \eta_{c}(1S, 2S)$ radiative transitions

Based on an integrated luminosity of $20.3~\mathrm{fb}^{-1}$ of $e^{+}e^{-}$ annihilation data collected at a center-of-mass energy of $3.773~\rm{GeV}$ with the BESIII detector operating at the BEPCII collider, an improved search for the radiative transitions $\psi(3770) \to \gamma \eta_{c}(1S, 2S)$ is performed using the hadronic decays $\eta_{c}(1S, 2S) \to K^{0}_{S} K^{\pm} \pi^{\mp}$. No significant signal is observed. The corresponding 90$\%$ confidence level upper limits on the product branching fractions are set to be $5.0 \times 10^{-6}$ for the $\eta_{c}(1S)$ transition and $3.7 \times 10^{-6}$ for the $\eta_{c}(2S)$ transition. The 90$\%$ confidence level upper limits on the partial decay widths are also reported to be $\Gamma(\psi(3770) \to \gamma \eta_{c}(1S)) < 5.5$ keV and $\Gamma(\psi(3770) \to \gamma \eta_{c}(2S)) < 29.4~\rm{keV}$. With about seven times larger integrated luminosity than used previously, these results lower the upper limits by approximately a factor of three and two for the $\eta_{c}(1S)$ and $\eta_{c}(2S)$ transitions, respectively.

==> acknowledgement_2026-05-25.tex <==
%% Saved at => 2026-05-25
\textbf{Acknowledgement}

The BESIII Collaboration thanks the staff of BEPCII (https://cstr.cn/31109.02.BEPC) and the IHEP computing center for their strong support. This work is supported in part by National Key R\&D Program of China under Contracts Nos. 2023YFA1606000, 2023YFA1606704, 2025YFA1613900; National Natural Science Foundation of China (NSFC) under Contracts Nos. 11635010, 11935015, 11935016, 11935018, 12025502, 12035009, 12035013, 12061131003, 12192260, 12192261, 12192262, 12192263, 12192264, 12192265, 12221005, 12225509, 12235017, 12342502, 12361141819, 12535005; the Chinese Academy of Sciences (CAS) Large-Scale Scientific Facility Program; the Strategic Priority Research Program of Chinese Academy of Sciences under Contract No. XDA0480600; CAS under Contract No. YSBR-101; 100 Talents Program of CAS; The Institute of Nuclear and Particle Physics (INPAC) and Shanghai Key Laboratory for Particle Physics and Cosmology; Agencia Nacional de Investigaci\'on y Desarrollo de Chile (ANID), Chile under Contract No. ANID CCTVal CIA250027; ERC under Contract No. 758462; German Research Foundation DFG under Contract No. FOR5327; Istituto Nazionale di Fisica Nucleare, Italy; Knut and Alice Wallenberg Foundation under Contracts Nos. 2021.0174, 2021.0299, 2023.0315; Ministry of Development of Turkey under Contract No. DPT2006K-120470; National Research Foundation of Korea under Contract No. RS-2026-25486791; National Science and Technology fund of Mongolia; Polish National Science Centre under Contract No. 2024/53/B/ST2/00975; STFC (United Kingdom); Swedish Research Council under Contract No. 2019.04595; U. S. Department of Energy under Contract No. DE-FG02-05ER41374

\textbf{Other Fund Information}

To be inserted with an additional sentence into papers that are relevant to the topic of special funding for specific topics. Authors can suggest which to Li Weiguo and/or the physics coordinator.
        Example added sentence: This paper is also supported by the NSFC under Contract Nos. 10805053, 10979059, ....National Natural Science Foundation of China (NSFC), 10805053, PWANational Natural Science Foundation of China (NSFC), 10979059, Lund弦碎裂强子化模型及其通用强子产生器研究National Natural Science Foundation of China (NSFC), 10775075, National Natural Science Foundation of China (NSFC), 10979012, baryonsNational Natural Science Foundation of China (NSFC), 10979038, charmoniumNational Natural Science Foundation of China (NSFC), 10905034, psi(2S)->B BbarNational Natural Science Foundation of China (NSFC), 10975093, D 介子National Natural Science Foundation of China (NSFC), 10979033, psi(2S)->VPNational Natural Science Foundation of China (NSFC), 10979058, hcNational Natural Science Foundation of China (NSFC), 10975143, charmonium rare decays
%% ends here %%


==> bibitem.tex <==
\begin{thebibliography}{99}

%%%%%%%%%%%%%%%%   Ref 1
\bibitem{Ref_admixture}J. L. Rosner, \href{https://doi.org/10.1103/PhysRevD.64.094002}{Phys. Rev. D {\bf 64}, 094002 (2001)}.

%%%%%%%%%%%%%%%%   Ref 2
\bibitem{Ref_obse1}P. A. Rapidis $et$ $al$., \href{https://doi.org/10.1103/PhysRevLett.39.526}{Phys. Rev. Lett. {\bf 39}, 526 (1977)}.

%%%%%%%%%%%%%%%%   Ref 3
\bibitem{Ref_obse2}W. Bacino $et$ $al$., \href{https://doi.org/10.1103/PhysRevLett.40.671}{Phys. Rev. Lett. {\bf 40}, 671 (1978)}.

%%%%%%%%%%%%%%%%   Ref 4
\bibitem{Ref_method1}M. Ablikim $et$ $al$. (BES Collaboration), \href{https://doi.org/10.1103/PhysRevLett.97.121801}{Phys. Rev. Lett. {\bf 97}, 121801 (2006)}.

%%%%%%%%%%%%%%%%   Ref 5
\bibitem{Ref_method2}M. Ablikim $et$ $al$. (BES Collaboration), \href{https://doi.org/10.1016/j.physletb.2006.08.049}{Phys. Lett. B {\bf 641}, 145 (2006)}.

%%%%%%%%%%%%%%%%   Ref 6
\bibitem{Ref_method3}M. Ablikim $et$ $al$. (BES Collaboration), \href{https://doi.org/10.1103/PhysRevD.76.122002}{Phys. Rev. D {\bf 76}, 122002 (2007)}.

%%%%%%%%%%%%%%%%   Ref 7
\bibitem{Ref_method4}M. Ablikim $et$ $al$. (BES Collaboration), \href{https://doi.org/10.1016/j.physletb.2007.11.078}{Phys. Lett. B {\bf 659}, 74 (2008)}.

%%%%%%%%%%%%%%%%   Ref 8
\bibitem{Ref_cleobf}D. Besson $et$ $al$. (CLEO Collaboration), \href{https://doi.org/10.1103/PhysRevLett.96.092002}{Phys. Rev. Lett. {\bf 104}, 159901(E) (2010)}.

%%%%%%%%%%%%%%%%   Ref 9
\bibitem{Ref_pdg}F. Takahashi $et$ $al$., \href{https://doi.org/10.1142/S0217751X26300115}{Int. J. Mod. Phys. A {\bf 41}, 2630011 (2026)}.

%%%%%%%%%%%%%%%%   Ref 
\bibitem{Ref_CLEO:2005zky}N. E. Adam $et$ $al$. (CLEO Collaboration), \href{https://doi.org/10.1103/PhysRevLett.96.082004}{Phys. Rev. Lett. {\bf 96}, 082004 (2006)}.

%%%%%%%%%%%%%%%%   Ref 
\bibitem{Ref_BESIII:2022yoo}M. Ablikim $et$ $al$. (BESIII Collaboration), \href{https://doi.org/10.1103/PhysRevD.107.L091101}{Phys. Rev. D {\bf 107}, L091101 (2023)}.

%%%%%%%%%%%%%%%%   Ref 
\bibitem{Ref_CLEO:2005zrs}G. S. Adams $et$ $al$. (CLEO Collaboration), \href{https://doi.org/10.1103/PhysRevD.73.012002}{Phys. Rev. D {\bf 73}, 012002 (2006)}.

%%%%%%%%%%%%%%%%   Ref 
\bibitem{Ref_BESIII:2023zsk}M. Ablikim $et$ $al$. (BESIII Collaboration), \href{https://doi.org/10.1103/PhysRevLett.132.131901}{Phys. Rev. Lett. {\bf 132}, 131901 (2024)}.

%%%%%%%%%%%%%%%%   Ref 
\bibitem{Ref_BESIII:2023rse}M. Ablikim $et$ $al$. (BESIII Collaboration), \href{https://doi.org/10.1007/JHEP11(2023)228}{JHEP {\bf 11}, 228 (2023)}.

%%%%%%%%%%%%%%%%   Ref 
\bibitem{Ref_BES:2006piq}M. Ablikim $et$ $al$. (BES Collaboration), \href{https://doi.org/10.1016/j.physletb.2007.06.074}{Phys. Lett. B {\bf 652}, 238 (2007)}.

%%%%%%%%%%%%%%%%   Ref 
\bibitem{Ref_BESIII:2015cby}M. Ablikim $et$ $al$. (BESIII Collaboration), \href{https://doi.org/10.1016/j.physletb.2015.11.074}{Phys. Lett. B {\bf 753}, 103 (2016)}.

%%%%%%%%%%%%%%%%   Ref
\bibitem{Ref_IML1}Y. J. Zhang, G. Li, and Q. Zhao, \href{https://doi.org/10.1103/PhysRevLett.102.172001}{Phys. Rev. Lett. {\bf 102}, 172001 (2009)}.

%%%%%%%%%%%%%%%%   Ref
\bibitem{Ref_IML2}F. K. Guo $et$ $al$., \href{https://doi.org/10.1103/PhysRevD.83.034013}{Phys. Rev. D {\bf 83}, 034013 (2011)}.

%%%%%%%%%%%%%%%%   Ref 13
\bibitem{Ref_IML3}G. Li, X. H. Liu, Q. Wang, and Q. Zhao, \href{https://doi.org/10.1103/PhysRevD.88.014010}{Phys. Rev. D {\bf 88}, 014010 (2013)}.

%%%%%%%%%%%%%%%%   Ref 10
\bibitem{Ref_iml}G. Li and Q. Zhao, \href{https://doi.org/10.1103/PhysRevD.84.074005}{Phys. Rev. D {\bf 84}, 074005 (2011)}.

%%%%%%%%%%%%%%%%   Ref 14
\bibitem{Ref_lqcd}J. J. Dudek, R. Edwards, and C. E. Thomas, \href{https://doi.org/10.1103/PhysRevD.79.094504}{Phys. Rev. D {\bf 79}, 094504 (2009)}.

%%%%%%%%%%%%%%%%   Ref 15
\bibitem{Ref_psi2}W. Li $et$ $al$., \href{https://doi.org/10.1103/PhysRevD.107.113002}{Phys. Rev. D {\bf 107}, 113002 (2023)}.

%%%%%%%%%%%%%%%%   Ref 16
\bibitem{Ref_LRC}S. Y. Pei $et$ $al$., \href{https://doi.org/10.1007/JHEP03(2026)153}{JHEP {\bf 03}, 153 (2026)}.

%%%%%%%%%%%%%%%%   Ref 17
\bibitem{Ref_3fb}M. Ablikim $et$ $al$. (BESIII Collaboration), \href{https://doi.org/10.1103/PhysRevD.89.112005}{Phys. Rev. D {\bf 89}, 112005 (2014)}.

%%%%%%%%%%%%%%%%   Ref 18
\bibitem{besiii}M. Ablikim $et$ $al$. (BESIII Collaboration), \href{https://doi.org/10.1016/j.nima.2009.12.050}{Nucl. Instrum. Meth. A {\bf 614}, 345 (2010)}.

%%%%%%%%%%%%%%%%   Ref 19
\bibitem{besiii2}K.-X. Huang $et$ $al$., \href{https://doi.org/10.1007/s41365-022-01133-8}{Nucl. Sci. Tech. {\bf 33}, 142 (2022)}.

%%%%%%%%%%%%   -- Ref 20
\bibitem{bepcii} C.~H.~Yu {\it et al.}, \href{https://accelconf.web.cern.ch/ipac2016/talks/tuya01_talk.pdf}{Proceedings of IPAC2016, Busan, Korea, 2016}.

%%%%%%%%%%%%   -- Ref 21
\bibitem{data1} J.~Lu, Y.~Xiao, and X.~Ji, \href{https://doi.org/10.1007/s41605-020-00188-8}{Rad. Det. Tech. Meth. {\bf 4}, 337 (2020)}.

%%%%%%%%%%%%   -- Ref 22
\bibitem{data2} J.-W.~Zhang {\it et al.}, \href{https://doi.org/10.1007/s41605-022-00331-7}{Rad. Det. Tech. Meth. {\bf 6}, 289 (2022)}.

%%%%%%%%%%%%   -- Ref 23
\bibitem{etof1} X.~Li {\it et al.}, \href{https://doi.org/10.1007/s41605-017-0014-2}{Rad. Det. Tech. Meth. {\bf 1}, 13 (2017)}.

%%%%%%%%%%%%   -- Ref 24
\bibitem{etof2} Y.~X.~Guo {\it et al.}, \href{https://doi.org/10.1007/s41605-017-0012-4}{Rad. Det. Tech. Meth. {\bf 1}, 15 (2017)}.

%%%%%%%%%%%%   -- Ref 25
\bibitem{etof3} P.~Cao {\it et al.}, \href{https://doi.org/10.1016/j.nima.2019.163053}{Nucl. Instrum. Meth. A {\bf 953}, 163053 (2020)}.

%%%%%%%%%%%%   -- Ref 26
\bibitem{G4} S. Agostinelli $et$ $al$. (GEANT4 Collaboration), \href{https://doi.org/10.1016/S0168-9002(03)01368-8}{Nucl. Instrum. Meth. A {\bf 506}, 250 (2003)}.

%%%%%%%%%%%%   -- Ref 27
\bibitem{kkmc} S.~Jadach, B.~F.~L.~Ward, and Z.~Was, \href{https://doi.org/10.1103/PhysRevD.63.113009}{Phys. Rev. D 63, 113009 (2001)}; \href{https://doi.org/10.1016/S0010-4655(00)00048-5}{Comput. Phys. Commun. {\bf 130}, 260 (2000)}.

%%%%%%%%%%%%   -- Ref 28
\bibitem{evtgen1} D. J.~Lange, \href{https://doi.org/10.1016/S0168-9002(01)00089-4}{Nucl. Instrum. Meth. A {\bf 462}, 152 (2001)}.

%%%%%%%%%%%%   -- Ref 29
\bibitem{evtgen2} R. G.~Ping, \href{https://doi.org/10.1088/1674-1137/32/8/001}{Chin. Phys. C {\bf 32}, 599 (2008)}.

%%%%%%%%%%%%   -- Ref 30
\bibitem{lundcharm1} J. C. Chen, G. S. Huang, X. R. Qi, D. H. Zhang, and Y. S. Zhu, \href{https://doi.org/10.1103/PhysRevD.62.034003}{Phys. Rev. D {\bf 62}, 034003 (2000)}.

%%%%%%%%%%%%   -- Ref 31
\bibitem{lundcharm2} R. L. Yang, R. G. Ping, and H. Chen, \href{https://doi.org/10.1088/0256-307X/31/6/061301}{Chin.\ Phys.\ Lett. {\bf 31}, 061301 (2014)}.

%%%%%%%%%%%%   -- Ref 32 
\bibitem{fsr} E. Barberio and Z. Was, \href{https://doi.org/10.1016/0010-4655(94)90074-4}{Comput. Phys. Commun. {\bf 79}, 291 (1994)}.

%%%%%%%%%%%%%%%%   Ref 33
\bibitem{Ref_vertexfit}M. Xu $et$ $al$., \href{https://doi.org/10.1088/1674-1137/34/1/017}{Chin. Phys. C {\bf 34}, 92 (2010)}.

%%%%%%%%%%%%%%%%   Ref 34
\bibitem{Ref_punzi}G. Punzi, \href{https://arxiv.org/abs/physics/0308063} {eConf C030908, MODT002 (2003)}.

%%%%%%%%%%%%%%%%   Ref 35
\bibitem{Ref_topo}X. Y. Zhou, S. X. Du, G. Li, and C. P. Shen, \href{https://doi.org/10.1016/j.cpc.2020.107540}{Comput. Phys. Commun. {\bf 258}, 107540 (2021)}.

%%%%%%%%%%%%%%%%   Ref 36
\bibitem{Ref_datadrive}M. Ablikim $et$ $al$. (BESIII Collaboration), \href{https://doi.org/10.1103/PhysRevD.111.052013}{Phys. Rev. D {\bf 111}, 052013 (2025)}.

%%%%%%%%%%%%   -- Ref 37
\bibitem{Ref_conexc}R. G. Ping, \href{https://doi.org/10.1088/1674-1137/38/8/083001}{Chin. Phys. C {\bf 38}, 083001 (2014)}.

%%%%%%%%%%%%   -- Ref 38
\bibitem{Ref_crosssection}B. Aubert $et$ $al$. (BaBar Collaboration), \href{https://doi.org/10.1103/PhysRevD.77.092002}{Phys. Rev. D {\bf 77}, 092002 (2008)}.

%%%%%%%%%%%%   -- Ref 39
\bibitem{Ref_isrpro}M. Benayoun $et$ $al$., \href{https://doi.org/10.1142/S021773239900273X}{Mod. Phys. Lett. A {\bf 14}, 2605 (1999)}.

%%%%%%%%%%%%   -- Ref 40
\bibitem{Ref_e7}N. Brambilla, Y. Jia, and A. Vairo, \href{https://doi.org/10.1103/PhysRevD.73.054005}{Phys. Rev. D {\bf 73}, 054005 (2006)}.

%%%%%%%%%%%%   Ref 41
\bibitem{Ref_damp}V. V. Anashin $et$ $al$. (KEDR Collaboration), \href{https://doi.org/10.1142/S2010194511000791}{Int. J. Mod. Phys. Conf. Ser. {\bf 02}, 188 (2011)}.

%%%%%%%%%%%%   Ref 42
\bibitem{Ref_signi}S. S. Wilks, \href{https://doi.org/10.1214/aoms/1177732360}{Ann. Math. Stat. {\bf 9}, 60 (1938)}.

%%%%%%%%%%%%   Ref 43
\bibitem{Ref_Bayesian}Y. Zhu, \href{https://doi.org/10.1016/j.nima.2007.05.116}{Nucl. Instrum. Meth. A {\bf 578}, 322 (2007)}.

%%%%%%%%%%%%%%%%   Ref 44
\bibitem{Ref_photon}M. Ablikim $et$ $al$. (BESIII Collaboration), \href{https://doi.org/10.1103/PhysRevD.81.052005}{Phys. Rev. D {\bf 81}, 052005 (2010)}.

%%%%%%%%%%%%%%%%   Ref 45
\bibitem{Ref_helixcor}M. Ablikim $et$ $al$. (BESIII Collaboration), \href{https://doi.org/10.1103/PhysRevD.87.012002}{Phys. Rev. D {\bf 87}, 012002 (2013)}.

%%%%%%%%%%%%%%%%   Ref 46
\bibitem{Ref_lum1}M. Ablikim $et$ $al$. (BESIII Collaboration), \href{https://doi.org/10.1088/1674-1137/37/12/123001}{Chin. Phys. C {\bf 37}, 123001 (2013)}.

%%%%%%%%%%%%%%%%   Ref 47
\bibitem{Ref_lum2}M. Ablikim $et$ $al$. (BESIII Collaboration), \href{https://doi.org/10.1088/1674-1137/ad70a0}{Chin. Phys. C {\bf 48}, 123001 (2024)}.

%%%%%%%%%%%%%%%%   Ref 48
\bibitem{Ref_bf1}M. Ablikim $et$ $al$. (BESIII Collaboration), \href{https://doi.org/10.1103/PhysRevD.100.012003}{Phys. Rev. D {\bf 100}, 012003 (2019)}.

%%%%%%%%%%%%%%%%   Ref 49
\bibitem{Ref_bf2}H. P. Wang and C. Z. Yuan, \href{https://doi.org/10.1088/1674-1137/ac5fa2}{Chin. Phys. C {\bf 46}, 071001 (2022)}.

%%%%%%%%%%%%%%%%   Ref 50
\bibitem{Ref_bf3}M. Ablikim $et$ $al$. (BESIII Collaboration), \href{https://doi.org/10.1103/PhysRevD.109.032004}{Phys. Rev. D {\bf 109}, 032004 (2024)}.

%%%%%%%%%%%%%%%%   Ref 
\bibitem{LHCb:2023evz}R. Aaij $et$ $al$. (LHCb Collaboration), \href{https://doi.org/10.1103/PhysRevD.108.032010}{Phys. Rev. D {\bf 108}, 032010 (2023)}.

%%%%%%%%%%%%%%%%   Ref 53
\bibitem{Ref_uplimit}K. Stenson, \href{https://doi.org/10.48550/arXiv.physics/0605236}{arXiv:physics/0605236 (2006)}.

%%%%%%%%%%%%%%%%   Ref 51
\bibitem{Ref_vacuum}S. Actis $et$ $al$. (Working Group on Radiative Corrections and Monte Carlo Generators for Low Energies), \href{https://doi.org/10.1140/epjc/s10052-010-1251-4}{Eur. Phys. J. C {\bf 66}, 585 (2010)}.

%%%%%%%%%%%%   -- Ref 52
\bibitem{Ref_radcor1} E.~A.~Kuraev and V.~S.~Fadin, \href{https://inis.iaea.org/records/pxvyx-wy164}{Sov. J. Nucl. Phys. {\bf 41}, 466 (1985)}.

\end{thebibliography}

